Predicting the Initial Conditions of the Universe using a Deterministic Neural Network

Finding the initial conditions that led to the current state of the universe is challenging because it involves searching over an intractable input space of initial conditions, along with modeling their evolution via tools such as N-body simulations which are computationally expensive. Recently, deep learning has emerged as a surrogate for N-body simulations by directly learning the mapping between the linear input of an N-body simulation and the final nonlinear output from the simulation, significantly accelerating the forward modeling. However, this still does not reduce the search space for initial conditions. In this work, we pioneer the use of a deterministic convolutional neural network for learning the reverse mapping and show that it accurately recovers the initial linear displacement field over a wide range of scales ($<1$-$2\%$ error up to nearly $k\simeq0.8$-$0.9 \text{ Mpc}^{-1}h$), despite the one-to-many mapping of the inverse problem (due to the divergent backward trajectories at smaller scales). Specifically, we train a V-Net architecture, which outputs the linear displacement of an N-body simulation, given the nonlinear displacement at redshift $z=0$ and the cosmological parameters. The results of our method suggest that a simple deterministic neural network is sufficient for accurately approximating the initial linear states, potentially obviating the need for the more complex and computationally demanding backward modeling methods that were recently proposed.

==> future_work.tex <==
% \section{Future Work}
% In this work, we showed that neural networks are successful in predicting the initial states of the N-body simulation at a wide range of scales, going down to small scales where nonlinear gravitational effects kick in. The inherent one-to-many mapping between the final states and the initial states at smaller scales makes it impossible for N-body simulators to make such predictions. However, inverse neural network models, such as the one presented in this work, can be trained to predict approximate initial states of N-body simulations which are correct for a wide range of scales. These approximate initial states could then be used as initializations by further downstream sampling-based methods (e.g. Hamiltonian Monte Carlo, Active Learning, etc.) to refine their search for better initial states which are correct at even smaller scales.

% Other directions for future work involve training on larger set of cosmological parameters, improving OOD performance, and uncertainty quantification for the initial states.

% % However, the ability to correctly make predictions at large scales can prove useful for sampling-based methods. Inverse models, such as the one presented in this work, can be trained to predict approximate initial states of N-body simulations which are correct at large scales. These approximate initial states could then be used as initializations for sampling-based methods that are commonly used.
